A Probabilistic Theory of Supervised Similarity Learning for Pointwise ROC Curve Optimization

The performance of many machine learning techniques depends on the choice of an appropriate similarity or distance measure on the input space. Similarity learning (or metric learning) aims at building such a measure from training data so that observations with the same (resp. different) label are as close (resp. far) as possible. In this paper, similarity learning is investigated from the perspective of pairwise bipartite ranking, where the goal is to rank the elements of a database by decreasing order of the probability that they share the same label with some query data point, based on the similarity scores. A natural performance criterion in this setting is pointwise ROC optimization: maximize the true positive rate under a fixed false positive rate. We study this novel perspective on similarity learning through a rigorous probabilistic framework. The empirical version of the problem gives rise to a constrained optimization formulation involving U-statistics, for which we derive universal learning rates as well as faster rates under a noise assumption on the data distribution. We also address the large-scale setting by analyzing the effect of sampling-based approximations. Our theoretical results are supported by illustrative numerical experiments.

==> parts/7-proofs.tex <==
% !TEX root = ../ICML_paper_supp.tex

% List of all of the propositions in this version of the paper
% ccl-slow-rates
% ccl-fast-rates  
 
% List of all of the propositions in the original note
% Positive U process universal rates
% * u-stat-plus
% * iid-plus
% * PAC-plus
% Negative U process universal rates
% * u-stat-minus
% * iid-minus
% * PAC-minus
% Universal rate conclusion
% * ccl-slow-rates
%
% Fast rates
% * var-control-1
% * var-control-2
% * bernstein
% * degen-U-stat
% * ccl-fast-rates
%\robin{To remove when sorted things with lemma 1.}

%\begin{proposition}
%Let $U_n$ be a U-statistic of degree 2 on some sample $(X_i)_{i=1}^n$ with kernel $H$ belongs to a family of kernels 
%Intermediary proposition about U-statistics with kernel of finite VC dimension.
%\end{proposition}
%With probability at least $1-\delta$,
%\begin{align*}
%\sup_{H \in \mathcal{H}} \abs{U_n - \E \left [ U_n \right ] } \le c \sqrt{\frac{V}{n}} 
%+ 2 \sqrt{\frac{ \log (1/\delta )}{n-1}} 
%\end{align*}

\subsection{Proof of \cref{ccl-slow-rates}}

The proof relies on the following argument from \citet[][Theorem~10 therein]{Clemencon2010} which points out that
\begin{align}
\begin{split}
  &\p \left\{\left\{ R^+ (\hat{S}_n)\ge \sup_{S \in \mathcal{S}_0 : \, R^-(S) \le \alpha } R^+(S)  
  -  C \Phi_{n,\delta/2} \right\} \cap   \left\{ R^- ( \hat{S}_n )\le \alpha + C \Phi_{n,\delta/2} \right\} \right\}\\
  &\ge 1 - \p\left\{ \sup_{ S \in\mathcal{S}_0 } \abs{R_n^+(S) - R^+(S)} > C\Phi_{n,\delta/2}  \right\} 
  - \p\left\{ \sup_{ S \in\mathcal{S}_0 } \abs{R_n^-(S) - R^-(S)} > C\Phi_{n,\delta/2}  \right\}.
  \end{split}
  \label{ineg-emp-proc}
\end{align}

Set $p =\sum_{k=1}^K p_k^2$ and observe that whe have: $\forall n>1$,
\begin{equation}
\sup_{ S \in\mathcal{S}_0 } \abs{R_n^+(S) - R^+(S)} \leq \frac{1}{p}\sup_{ S \in\mathcal{S}_0 } \abs{U_n^+(S) - \E \left [ U_n^+(S) \right ]} +\frac{2n_+/(n(n-1))-p}{p(p+2n_+/(n(n-1))-p)}
\end{equation}
as well as
\begin{equation}
\sup_{ S \in\mathcal{S}_0 } \abs{R_n^-(S) - R^-(S)} \leq \frac{1}{1-p}\sup_{ S \in\mathcal{S}_0 } \abs{U_n^-(S) - \E \left [ U_n^-(S) \right ]} +\frac{2n_-/(n(n-1))-(1-p)}{(1-p)(1-p+2n_-/(n(n-1))-(1-p))}.
\end{equation}
Hence, combining Lemma \ref{lem:Ubounds} with the variant of Hoeffding's inequality for U-statistics (see \textit{e.g.} Theorem A of section 5.6 in \cite{Ser80})) applied to the $U$-statistics $2n_+/(n(n-1))$ and $2n_-/(n(n-1))$ yields bounds for $\sup_{ S \in\mathcal{S}_0 } \abs{R_n^+(S) - R^+(S)}$ and $\sup_{ S \in\mathcal{S}_0 } \abs{R_n^-(S) - R^-(S)} $ of the same order as that stated in Eq. \eqref{eq:Ubounds}. The proof is then finished by following line by line the proof of Theorem 10 in \cite{Clemencon2010}.

%Using \cref{lem:Ubounds} and standard results for U-statistics, \robin{cite Hoeffding or "Ranking and ERM 
%of U-statistics"}, with probability at least $1-\delta$,
%\begin{align*}
%\sup_{S\in \mathcal{S}} \abs{ U_n^+(S) - \E \left [ U_n^+(S) \right ]} &\le 
%4c \sqrt{\frac{V}{n}} + 4 \sqrt{\frac{ \log (2/\delta )}{n-1}} \\
%\abs{ \frac{2n_+ }{n(n-1)} - p }
%&\le  \sqrt{\frac{\log  \left ( 2 / \delta \right ) }{n-1}}\\
%\end{align*}
%When $n \ge 1 + 4 \log \left ( 2/\delta \right )/p^2$, 
%we have $\abs{ \frac{2n_+ }{n(n-1)p} - 1 } \le 1/2$ and therefore that
%\begin{align*}
%\abs{ \frac{n(n-1)p}{2n_+ } - 1 } & \le 2 \abs{ \frac{2n_+}{n(n-1)p} - 1   }  \\
%& \le 2 p^{-1} \sqrt{\frac{\log  \left ( 2 / \delta \right ) }{n-1}} \\
%\end{align*}
%since $x \mapsto 1/x$ is convex on $\R_+$. Using $\frac{ n(n-1)  }{2n_+} =  
% \left ( \frac{ n(n-1)  }{2n_+} - p^{-1 } \right ) + p^{-1}$, it implies that
%\begin{align*}
%\sup_{S\in \mathcal{S}} \abs{ \frac{ n(n-1) U_n^+(S) }{2n_+} - R_+(S)  } &\le 
% \abs{ \left (  \frac{ n(n-1)  }{2n_+} - p^{-1} \right )} \sup_{S\in \mathcal{S}} \abs{ U_n^+(S)} +
%p^{-1}\sup_{S\in \mathcal{S}} \abs{  U_n^+(S) - \E \left [ U_n^+(S) \right ] }\\
%&\le p^{-1} \left [  4c \sqrt{\frac{V}{n}} + 6 \sqrt{\frac{ \log (2/\delta )}{n-1}}  \right ]
%\end{align*}
%which gives the result.
%
%%Similarly, when $n \ge 1 + 4 \log \left ( 2/\delta \right )/ (1-p)^2$, 
%with probability at least $1-\delta$, 
%\begin{align*}
%\sup_{S\in \mathcal{S}} \abs{ \frac{ n(n-1) U_n^-(S) }{2n_-} - R_-(S)  } 
%&\le (1-p)^{-1} \left [  4 c \sqrt{\frac{V}{n}} + 6 \sqrt{\frac{ \log (2/\delta )}{n-1}}  \right ]
%\end{align*}
%
%%Since $p^{-1} \le \kappa^{-1}$ and $(1-p)^{-1} \le \kappa^{-1}$, taking $C = \kappa^{-1}$ and 
%\begin{align}
%\Phi_{n, \delta} = 4c \sqrt{\frac{V}{n}} + 6 \sqrt{\frac{\log (2/\delta)}{n-1}}
%\end{align}
%concludes the proof. 


\subsection{Proof of \cref{ccl-fast-rates}}
Set $S^*(x,x')=\mathbb{I}\{(x,x')\in\mathcal{R}^*_{\alpha} \}$ be the optimal similarity function (supposed here to belong to $\mathcal{S}_0$ for simplicity).
Observe that, for any $S\in \mathcal{S}$, the statistic 
\begin{equation}\label{eq:deltaU}
\Delta_{n} (S) = \left ( U_n^+(S) - \E \left [ U_n^+(S) \right ] \right ) 
- \left ( U_n^+(S^*) - \E \left [ U_n^+(S^*) \right ] \right )
\end{equation}
is a U-statistic based on $\mathcal{D}_n$ with kernel $Q_S$ given by
\begin{align*}
Q_S((x,y),(x',y')) &= \I\left \{ y=y' \right \} \left ( S(x,x')-S^*(x,x')\right ) 
- \E \left [ \I\left \{ Y=Y' \right \} \left ( S(X,X') - S^*(X,X') \right ) \right ] 
\end{align*}
The proof relies on the second Hoeffding decomposition of $U$-statistics, already used for the fast rate analysis carried out in \cite{Clemencon08Ranking} in ranking risk minimization, which claims that the $U$-statistics \eqref{eq:deltaU} can be decomposed as follows
\begin{equation}\label{eq:decomp}
\Delta_{n}(S) = 2 T_n(S)  + W_n(S) ,
\end{equation}
where 
\begin{equation*}
T_n (S)= \frac{1}{n} \sum_{i=1}^n q_S (X_i,Y_i) \text{ and } W_n(S) = \frac{2}{n(n-1)} \sum_{1 \le i < j \le n} \widehat{q}_S \left ((X_i, Y_i), (X_j , Y_j) \right ) ,
\end{equation*}
with 
\begin{align*}
q_S (x,y) &= \E \left [ Q_S\left ( (X, Y), (x, y) \right ) \right ] \\
\widehat{q}_S \left ( (x,y),(x',y') \right ) &= 
Q_S \left ( (x, y) , (x',y' ) \right ) - q_S (x,y) - q_S (x',y').
\end{align*}
The component $W_n(S)$ is a degenerate $U$-statistic, meaning that, for all $(x,y)$, $$\mathbb{E}\left[\widehat{q}_S \left ( (x,y),(X,Y) \right )\right]=0 \text{ almost-surely.}$$
The following lemma is thus a direct consequence of the bound established in \cite{ArconesGine}.
\begin{lemma}
Suppose that the hypotheses of Theorem \ref{ccl-fast-rates} are fulfilled. 
The, for any $\delta\in (0,1)$, we have with probability larger than $1-\delta$: $\forall n\geq 2$,
 $$
 \sup_{S\in \mathcal{S}_0}\left\vert W_n(S) \right\vert \leq C\times \frac{V\log(n/\delta)}{n},
 $$
 where $C<+\infty$ is a universal constant.
 \end{lemma}
 This result shows that the second term in decomposition \eqref{eq:decomp} is uniformly negligible with respect to $T_n(S)$. The ingredient is the following lemma, which provides a control of the variance of $T_n(S)$ under the {\bf NA} condition.
 \begin{lemma} Suppose that the hypotheses of Theorem \ref{ccl-fast-rates} are fulfilled. Then, for any $S\in \mathcal{S}_0$, we have:
 \begin{equation*}
\text{Var} (q_S(X,Y)) 
\le  c \left [ (1-Q^*_\alpha) p ( R^+ (S^*) - R^+ (S) ) + (1-p) Q^*_\alpha (R^-(S) - R^-(S^*) ) \right ]^a \\
 \end{equation*}
 \label{var-control-1-old}
 \end{lemma}
 It is the analogue of Lemma 11 in \cite{Clemencon2010} and the fast rate bound stated in Theorem \ref{ccl-fast-rates} then classically follows from the application of Talagrand's inequality (or Bernstein's inequality when $\mathcal{S}_0$ is of finite cardinality, see \textit{e.g.} subsection 5.2 in \cite{Boucheron2005}, just like that stated in Theorem 12 in \cite{Clemencon2010}.
 
%The bound over $R_n^+(S)$ minus its expectancy will be refined using Bernstein's inequality, thus we
%need to control $\text{Var} \left ( q (X,Y)\right )$. An equivalent of the noise condition proven in 
%\cite{Bousquet2004} is the following condition
%\begin{align*} %
%\exists c > 0, \; \forall A \subset \X \times \X, \quad  \p \left( X,X'\in A \right) 
%\le c \left ( \int_A \abs{\eta(X,X') - Q^*_\alpha } \; d \, \p_{X,X'}(x,x') \right )^a
%\end{align*}
%
%\begin{proposition}
%\begin{align*}
%\text{Var} (q(X,Y)) & \le  c \left ( \int_0^1 \E \left [ \I\left\{ X,X' \in R_{S,u} \Delta R^*_\alpha  \right\}
%\abs{ \eta(X,X') - Q^*_\alpha } \right ] \; du \right )^a \\
%\end{align*}
%\label{var-control-1}
%\end{proposition}
%
%\begin{proof}
%The second moment bound gives
%\begin{align*}
%\text{Var} (q(X,Y))  &= 
%\E_{X,Y} \left [ \left ( \E_{X',Y'} \left [ \I\left \{ Y = Y' \right \} 
%\left ( S(X,X')-S^*(X,X') \right ) \right ]\right )^2  \right ] \\
%&\le \E \left [  \I\left \{ Y = Y' \right \} 
%\left ( S(X,X')-S^*(X,X')  \right )^2  \right ] \\
%& \le  \E \left [  \I\left \{ Y = Y' \right \} \abs{ S(X,X')-S^*(X,X')   }  \right ]
%\end{align*}
%since $\abs{ S(X,X')-S^*(X,X')} \le 1$.
%We introduce the following notations
%\begin{align*}
%R^*_\alpha &:= \left \{ x,x' \in \X\times \X \, | \, \eta(x,x') > Q^*_\alpha \right \} \\
%R_{S,u} &:=    \left \{ x,x' \in \X\times \X \, | \, S(x,x') > u \right \} \\
%\end{align*}
%We can always write the value $S(X,X')$ as the integral of $ u \mapsto \I_{ R_{S,u}} (X,X')$ on $[0,1]$.
%Under the noise condition, we have that $s^* = \I_{R^*_\alpha}$. By Jensen's inequality
%\begin{align*}
%\text{Var} (q(X,Y)) & \le  \int_0^1 \E \left [  \I\left \{ Y \ne Y' \right \} 
%\abs{ \I_{ R_{S,u}}(X,X')- \I_{R^*_\alpha}(X,X')   }  \right ] \; du \\
% & \le  \int_0^1 \E \left [  \abs{ \I_{ R_{S,u} \Delta R^*_\alpha }(X,X') }  \right ] \; du \\
%\end{align*}
%By the corollary of the noise condition, followed by Jensen's inequality
%\begin{align*}
%\text{Var} (q(X,Y)) & \le  \int_0^1 \p \left ( X,X' \in R_{S,u} \Delta R^*_\alpha \right ) \; du \\
%& \le  c \left ( \int_0^1 \E \left [ \I\left\{ X,X' \in R_{S,u} \Delta R^*_\alpha  \right\}
%\abs{ \eta(X,X') - Q^*_\alpha } \right ] \; du \right )^a \\
%\end{align*}
%\end{proof}
%
%\begin{proposition}
%\begin{align*}
%\text{Var} (q(X,Y)) & 
%\le  c \left [ (1-Q^*_\alpha) p ( R^+ (S^*) - R^+ (S) ) + (1-p) Q^*_\alpha (R^-(S) - R^-(S^*) ) \right ]^a \\
%\end{align*}
%\end{proposition}
%
%\begin{proof}
%Using that
%\begin{align*}
%\left (  \I_{R_{s,u}}(X,X') - \I_{R^*_\alpha} (X,X') \right ) 
%\left ( \eta(X,X') - Q^*_\alpha \right ) = - \I_{R_{s,u} \Delta R^*_\alpha}(X,X') \abs{\eta(X,X') - Q^*_\alpha }
%\end{align*}
%we obtain
%\begin{align*}
%R^+(S)-R^+(S^*) &= \int_{[0,1]} \E \left [ \I_{R_{s,u}}(X,X') - \I_{R^*_\alpha} (X,X')  | Z = +1 \right ] \; du \\
%&= p^{-1}  \int_{[0,1]} \E \left [ \left (  \I_{R_{s,u}}(X,X') - \I_{R^*_\alpha} (X,X') \right ) \eta(X,X') \right ] 
%\; du \\
%&= p^{-1}  \int_{[0,1]} \E \left [ \left (  \I_{R_{s,u}}(X,X') - \I_{R^*_\alpha} (X,X') \right ) 
%\left ( \eta(X,X') - Q^*_\alpha \right ) \right ] \; du \\
%& \quad + p^{-1} Q^*_\alpha \int_{[0,1]} 
%\E \left [ \left (  \I_{R_{s,u}}(X,X') - \I_{R^*_\alpha} (X,X') \right ) \right ] \; du \\
%&= - p^{-1}  \int_{[0,1]} \E \left [ \I_{R_{s,u} \Delta R^*_\alpha}(X,X') \abs{\eta(X,X') - Q^*_\alpha } \right ] 
%\; du \\
%& \quad +  Q^*_\alpha  \left ( R^+(S)-R^+(S^*)\right ) + p^{-1} Q^*_\alpha (1-p) \left ( R^-(S)-R^-(S^*)\right )
%\end{align*}
%Multiplying by $p$ and rearranging the terms gives
%\begin{align*}
% \int_{[0,1]} \E \left [ \I_{R_{s,u} \Delta R^*_\alpha}(X,X') \abs{\eta(X,X') - Q^*_\alpha } \right ] \; du &= 
% p \left ( 1-Q^*_\alpha \right )\left ( R^+(S^*) - R^+(S) \right ) +  (1-p) Q^*_\alpha \left ( R^-(S)-R^-(S^*)\right )
%\end{align*}
%Combining with \cref{var-control-1} gives the result.
%\end{proof}
%
%\begin{align*}
%\p \left ( \Delta_n(S) > t  \right ) & \le \p \left( 4T_n(S) > t \right ) + \p \left ( 2W_n > t \right )
%\end{align*}
%
%Results on degenerate U-statistics give that,
%\begin{align*}
%\p \left ( W_n(S) > u \right ) & \le L
%\end{align*}
%
%\robin{Something better for $W_n$.}
%
%Bernstein's inequality states that, since $\abs{q}\le 2$
%\begin{align*}
%\p \left ( T_n(S) > u  \right ) & \le \exp \left ( - \frac{n u^2}{2 \text{Var} \left( q(X,Y) \right )  + 4u/3}\right ) 
%\end{align*}
%hence 
%\begin{align*}
%\p \left ( 4 T_n(S) > t \right ) & \le \exp \left ( - \frac{n t^2}
%{32 \text{Var} \left( q(X,Y) \right )  + 16 t/3}\right ) 
%\end{align*}
%
%\begin{align*}
%\p \left ( \Delta_n(S) > t  \right ) & \le 2 
%\max \left (\exp \left ( - \frac{n t^2}
%{32 \text{Var} \left( q(X,Y) \right )  + 16 t/3}\right ) 
% , \dots  \right )
%\end{align*}
%When $n$ is big enough, the dominant term is the left hand side one, hence \dots


\subsection{Proof of \cref{prop:var}}
Conditioned upon the $(Y_i)_{i=1}^n$, the sample $\left ( X_i, Y_i \right )_{i=1}^n$ is seen as $K$ samples 
$\left ( X_{i_k} \right )_{i_k=1}^{n_k}$, $k \in \{ 1, \dots , K\}$, one for each class, and
$R_n^-(S)$ can be written as a $K$-sample $U$-statistic with kernel $h_S$. Indeed,
\begin{align*}
R_n^-(S) &= \frac{1}{n_-} \sum_{k<l} 
\sum_{ i_{k} = 1}^{n_k} \sum_{i_l=1}^{n_l} S \left ( X_{i_k}, X_{i_l} \right ), \\
 &=  \frac{1}{\prod_{k=1}^K n_k }\sum_{ i_{1} = 1}^{n_1}  \dots  \sum_{ i_{K} = 1}^{n_K}  
   \sum_{k<l}  \frac{n_k n_l}{n_-} S \left ( X_{i_k}, X_{i_l} \right ), \\
    &=  \frac{1}{\prod_{k=1}^K n_k }\sum_{ i_{1} = 1}^{n_1}  \dots  \sum_{ i_{K} = 1}^{n_K}  
    h_S \left ( X_{i_1} , \dots, X_{i_K} \right ).\\
\end{align*}

From \citet[][Equation~(21) therein]{JMLRincompleteUstats}, we have that
\begin{align*}
\text{Var}\left ( \widetilde{R}_B^- (S) \right ) &= 
\left( 1 - \frac{1}{B} \right) \text{Var} \left ( R_n^-(S)\right ) 
+ \frac{1}{B} \text{Var} \left ( h_S \left ( X^{(1)} , \dots , X^{(K)} \right ) \right ),
\end{align*}
which gives the result for tuple-based sampling since 
$\text{Var}\left ( R_n^-(S) \right ) = O \left ( 1 / n \right )$ when $B_0/n \to 0$, $n\to \infty$
 and $n_k/n \to p_k > 0$ for all $k\in\{1,\dots, K \}$. 
 
Straightforwardy adapting the proof of \citet[][Equation~(21) therein]{JMLRincompleteUstats} for the case of 
pair-based sampling gives
\begin{align*}
\text{Var} \left ( \bar{R}_B^-(S) \right )  &=  \left ( 1 - \frac{1}{B} \right ) \text{Var} \left ( R_n^-(S) \right )
+ \frac{1}{B} \left [  \sum_{k<l}  \frac{n_k n_l}{n_-} \E \left [S^{2} \left ( X^{(k)}, X^{(l)} \right )\right ] 
- \left ( \sum_{k<l} \frac{n_k n_l}{n_-} \E \left [ S \left ( X^{(k)}, X^{(l)} \right )\right ] \right )^2 \right ],
\\
 &=  \left ( 1 - \frac{1}{B} \right ) \text{Var} \left ( R_n^-(S) \right )
+ \frac{1}{B} \text{Var} \left ( S \left ( X,X' \right ) \, | \, Y \ne Y' \right ).  \\
\end{align*}


\begin{comment}

\subsection{Proof of Theorem 5 in \cite{Clemencon08Ranking}}

\subsubsection{Understanding the role of \citet[][Theorem~11]{Clemencon08Ranking} in \citet[][Theorem~5]{Clemencon08Ranking}}
Using the notations of the paper, Theorem 11 is claimed to imply that: with probability at least $1-\delta/2$,  $\sup_{r \in \mathcal{R}} \abs{W_n(r)} \le \kappa$, where
\begin{align*}
\kappa = C \left ( \frac{\E Z_\epsilon }{n(n-1)} + \frac{\E U_\epsilon \sqrt{\log(2/\delta)}}{n(n-1)} + \frac{\E M \log(2/\delta)}{n(n-1)} + 4 \frac{\log(2/\delta)}{n-1} \right ),
\end{align*}
and $C$ is an appropriate constant. 

\robin{Modified kappa denominators, necessary for $\E Z_\epsilon$, others for prettiness.
Modified also the $1/\delta$ to $2/\delta$, and added a 4 in front of $\frac{\log(2/\delta)}{n-1}$ since otherwise it is harder to conclude.}

Note that $\{ \hat{h}_r \mid r \in \mathcal{R} \}$ is a class of kernels and that $\E [ \hat{h}_r((X,Y),(x,y)) ] = 0$ and $\hat{h}_r((x,y),(x,y)) = 0$ for all $x,y$.
The second point comes from the fact that the ranking rules are considered symmetric, see \citet[][bottom page~851]{Clemencon08Ranking}.
Then if $\mathcal{F} := \{ \hat{h}_r \mid r \in \mathcal{R} \}$, from the definition of $Z$, $Z = n(n-1)\sup_{r \in \mathcal{R}} \abs{W_n(r)}$ and it follows that,
\begin{align*}
\p \left \{ n(n-1)\sup_{r \in \mathcal{R}} \abs{W_n(r)} > C \E Z_\epsilon + t  \right \} &\le \exp 
\left ( - \frac{1}{C} \min \left ( \left( \frac{t}{\E U_\epsilon } \right )^2 ,
 \frac{t}{\E M + Fn }, \left ( \frac{t}{F\sqrt{n}} \right )^{2/3} , \sqrt{\frac{t}{F}} \right ) \right ).
\end{align*}
To derive a lower bound on $\sup_{r \in \mathcal{R}} \abs{W_n(r)}$ with probability $1-\delta/2$, it then suffices to show that,
\begin{align*}
 \exp \left ( - \frac{1}{C} \min \left ( \left( \frac{t}{\E U_\epsilon } \right )^2 ,
 \frac{t}{\E M + Fn }, \left ( \frac{t}{F\sqrt{n}} \right )^{2/3} , \sqrt{\frac{t}{F}} \right ) \right )
 &\le \delta/2.
\end{align*}
It is equivalent to,
\begin{align*}
 \min \left ( \left( \frac{t}{\E U_\epsilon } \right )^2 ,
 \frac{t}{\E M + Fn }, \left ( \frac{t}{F\sqrt{n}} \right )^{2/3} , \sqrt{\frac{t}{F}} \right ) 
  &\ge C \log(2/\delta),
\end{align*}
and hence to having all four inequalities:
\begin{align*}
t &\ge \sqrt{C \log(2/\delta)} \cdot \E U_\epsilon, \\
t &\ge C \log (2/\delta) \left ( \E M + Fn  \right ),  \\
t &\ge \left(C \log (2/\delta)\right)^{3/2} F \sqrt{n}, \\
t &\ge \left(C \log (2/\delta)\right)^{2} F . \\
\end{align*}
In our case, we expect the bound when $ C\E Z_\epsilon + t  = \kappa n(n-1)$ which is equivalent to:
\begin{align*}
t = C \left (  \E U_\epsilon \sqrt{\log(2/\delta)} + \E M \log(2/\delta) + 4 n \log(2/\delta) \right ) .
\end{align*}
The first inequality is trivial, the second one follows from $F \le 4$ and the last ones only seem to be true when $n$ is large.
It follows from $\abs{q_r} \le 1$ that $F\le 4$, since  
\begin{align*}
\abs{\hat{h}_r((x,y),(x',y'))} &= \abs{q_r((x,y),(x',y')) + \Lambda(r) -  \E q_r((x,y),(X',Y')) - \E q_r((x',y'),(X,Y))}, \\
&\le 4,
\end{align*}
which concludes the proof.

\subsubsection{Part between the use of Theorem 11 and Massart's property}
Note that $\ell (r,(x,y)) - \ell (r^*, (x,y)) = 2 h_r (x,y) + \Lambda(r)$, it follows that
\begin{align*}
2T_n(r) &= \frac{1}{n} \sum_{i=1}^n \ell (r,(X_i,Y_i)) - \frac{1}{n} \sum_{i=1}^n \ell (r^*,(X_i,Y_i))  - \Lambda(r), \\
\Lambda_n(r) &=  \frac{1}{n} \sum_{i=1}^n \ell (r,(X_i,Y_i)) - \frac{1}{n} \sum_{i=1}^n \ell (r^*,(X_i,Y_i))  + W_n(r). \\
\end{align*}
Hence: $\forall r \in \mathcal{R}$, $\Lambda_n(r_n) \le \Lambda_n(r)$ which gives that, on the event $A$,
\begin{align*}
\forall r \in \mathcal{R}, \qquad \frac{1}{n} \sum_{i=1}^n \ell ( r_n,  (X_i,Y_i)) &\le \frac{1}{n} \sum_{i=1}^n \ell (r , (X_i,Y_i)) + (W_n(r) - W_n(r_n)), \\
&\le \frac{1}{n} \sum_{i=1}^n \ell (r,  (X_i,Y_i)) + 2 \kappa,\\
\end{align*}
which proves that $r_n$ is a $2\kappa$-minimizer of $(1/n)\sum_{i=1}^n \ell (r, (X_i,Y_i))$ on $A$.
The definition of $\widetilde{r}_n$ and the properties that it has don't need further detail.

\subsubsection{Use of \citet[][Theorem~8.3 therein]{Massart2006}}
We introduce the equivalent of the paper's notations,
\begin{itemize}
\item $\xi_1, \dots, \xi_n \; \to ((X_1,Y_1), \dots, (X_n,Y_n))$,
\item $\gamma(t,x) \; \to \ell(r, (x,y))$,
\item $\ell(s,t) \; \to \E \ell(r,(X,Y)) - \E \ell (r^*,(X,Y)) = \Lambda (r)$,
\item $\gamma_n(t) \; \to \frac{1}{n} \sum_{i=1}^n \ell(r,(X_i,Y_i))$,
\item $\bar{\gamma}_n(t) \; \to \frac{1}{n} \sum_{i=1}^n \ell(r,(X_i,Y_i)) - \E \ell(r, (X,Y))$.
\end{itemize}
\citet[][Equation~(8.16) therein]{Massart2006} writes,
\begin{align*}
\E \left [ \left( \ell(r, (X,Y)) - \ell(r^*,(X,Y)) \right)^2 \right ] &\le d^2(r,r^*),\\
\E_{X,Y} \left [ \left( 2 \E_{X',Y'} \left [ \I\{ (Y-Y')r(X,X') < 0 \} -  \I\{ (Y-Y')r^*(X,X') < 0 \} \right ]  \right)^2 \right ] &\le d^2(r,r^*). \\
\end{align*}
Since, by Jensen's inequality, 
\begin{align*}
\abs{\E_{X',Y'} \left [ \I\{ (Y-Y')r(X,X') < 0 \} -  \I\{ (Y-Y')r^*(X,X') < 0 \} \right ] } \le \E_{X',Y'} \left [ \I\{ r(X,X') \ne r^*(X,X')  \} \right ],
\end{align*}
It follows that,
\begin{align*}
\E \left [ \left( \ell(r, (X,Y)) - \ell(r^*,(X,Y)) \right)^2 \right ] &\le 4 \E_{X,Y} \left [ \left( \E_{X',Y'} \left [ \I\{ r(X,X') \ne r^*(X,X')  \} \right ] \right)^2 \right ] , \\
&\le 4 d^2(r,r^*), \\
\end{align*}
add \citet[][Equation~(8.16) therein]{Massart2006} is true, up to a constant.

\citet[][Equation~(8.17) therein]{Massart2006} writes,
\begin{align*}
d(r,r^*) \le w \left ( \sqrt{\Lambda(r)} \right ),
\end{align*}
where $w$ is some function. Note that $\Lambda (r) = \E [\I\{r(X,X') \ne r^*(X,X') \} \abs{\eta(X)- \eta(X')}]$. 
We believe that this condition will necessite the use of the noise condition, i.e. \citet[][Assumption~4 therein]{Clemencon08Ranking}.
However, it would require us to lower-bound $\text{Var} \left ( h_r (X,Y) \right )$ by $d(r,r^*)$. \robin{Got stuck here.}


\citet[][Equation~(8.18) therein]{Massart2006} writes, for every $r_0 \in \mathcal{R}$,
\begin{align*}
\sqrt{n} \E \left [ \sup_{r \in \mathcal{R} , d(r,r_0) \le \sigma } \abs{ 
\left ( \frac{1}{n} \sum_{i=1}^n \ell(r,(X_i,Y_i)) - \E \ell(r,(X,Y)) \right )  - 
\left ( \frac{1}{n} \sum_{i=1}^n \ell(r_0,(X_i,Y_i)) - \E \ell(r_0,(X,Y)) \right )  } \right ] &\le \phi(\sigma), \\
\sqrt{n} \E \left [ \sup_{r \in \mathcal{R} , d(r,r_0) \le \sigma } \abs{ 
 \frac{1}{n} \sum_{i=1}^n \ell(r,(X_i,Y_i)) - \frac{1}{n} \sum_{i=1}^n \ell(r_0,(X_i,Y_i))  } \right ] &\le \phi(\sigma), \\
\end{align*}

\subsubsection{Proof of \citet[][Proposition~7]{Clemencon08Ranking}}

Note that, in the case of bipartite ranking with a scorer, we have that,
\begin{align*}
q_r ((x,y),(x',y')) &= \I\{ (y-y') (s(x) - s(x')) < 0\} - \I\{ (y-y') ( \eta (x) - \eta (x')) < 0\},\\
&= \I\{  (s(x) - s(x')) (\eta(x) - \eta (x')) < 0\} \left ( \I\{Y \ne Y' \}  - 2 \I\{(\eta(x)-\eta(x')) (y-y') < 0\}  \right ) .
\end{align*}
Hence,
\begin{align*}
\E[q_r ((X,Y),(X',Y')) \mid X=x,X'=x'] &= \I\{  (s(x) - s(x')) (\eta(x) - \eta (x')) < 0\}  \abs{\eta(x)-\eta(x')},
\end{align*}
which implies that
\begin{align*}
\Lambda(r) &=  \E \left [  \abs{ \eta(X)  - \eta(X') } 
\I\{  \left ( s(X)-s(X') \right  ) \left ( \eta(X)-\eta(X') \right  )  < 0\}  \right ] \\
\end{align*}
Hence, since $h_s (x,y) = \E q_r ((x,y) , (X',Y')) - \Lambda(r)$, then
\begin{align*}
\text{Var} \left ( h_s(X,Y) \right ) & \le 
\E_{X,Y}  \left [ \left ( \E_{X',Y'} [ q_r ((X,Y) , (X',Y'))]  \right )^2\right ], \\
& \le \E_X  \left [ \left ( \E_{X'} \left ( \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]} \right )  \right )^2\right ], \\
\end{align*}
Consider the scalar product $\langle \cdot, \cdot , \rangle$ that satisfies, $\langle f,g \rangle = \E_{X'} [fg]$,
the associated Cauchy-Schwartz gives
\begin{align*}
& \left ( \E_{X'} \left ( \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]}  \right )  \right )^2, \\
& \quad = \left ( \E_{X'} \left ( \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]} 
\abs{\eta(X)-\eta(X')}^{\alpha/2} \abs{\eta(X)-\eta(X')}^{-\alpha/2} \right )  \right )^2, \\
& \quad \le \E_{X'}  \left [  \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]} \abs{\eta(X)-\eta(X')}^{\alpha} \right ] 
 \E_{X'}  \left [  \abs{\eta(X)-\eta(X')}^{ - \alpha} \right ] .\\
\end{align*}
Hence,
\begin{align*}
\text{Var} \left ( h_s(X,Y) \right ) & \le \E_X  \left [ \left ( \E_{X'} \left ( \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]} \abs{\eta(X)-\eta(X')}^{\alpha} \right )  \right )  
\left ( \E_{X'} \left (  \abs{\eta(X)-\eta(X')}^{-\alpha} \right )  \right )\right ], \\
& \text{(Cauchy-Schwartz)}\\
& \le c \E_X  \left [ \left ( \E_{X'} \left ( \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]} 
\abs{\eta(X)-\eta(X')}^{\alpha} \right )  \right )  \right ], \\
& \text{(Noise assumption)}\\
& \le c \E_{X,X'} \left [ \I_{[(s(X)-s(X'))(\eta(X)-\eta(X')) < 0]} 
\abs{\eta(X)-\eta(X')} \right ]^{\alpha}, \\
& \text{(Jensen inequality)}\\
& \le c \Lambda (r)^{\alpha}, \\
\end{align*}

\end{comment}



